Parameter Database : Data-centric Synchronization for Scalable Machine Learning

We propose a new data-centric synchronization framework for carrying out of machine learning (ML) tasks in a distributed environment. Our framework exploits the iterative nature of ML algorithms and relaxes the application agnostic bulk synchronization parallel (BSP) paradigm that has previously been used for distributed machine learning. Data-centric synchronization complements function-centric synchronization based on using stale updates to increase the throughput of distributed ML computations. Experiments to validate our framework suggest that we can attain substantial improvement over BSP while guaranteeing sequential correctness of ML tasks.

==> nips-bib.tex <==
@inproceedings{li_pserver,
  title={Scaling distributed machine learning with the parameter server},
  author={Li, Mu and Andersen, David G and Park, Jun Woo and Smola, Alexander J and Ahmed, Amr and Josifovski, Vanja and Long, James and Shekita, Eugene J and Su, Bor-Yiing},
  booktitle={Proc. OSDI},
  pages={583--598},
  year={2014}
}

@inproceedings{cipar2013solving,
  title={Solving the straggler problem with bounded staleness},
  author={Cipar, James and Ho, Qirong and Kim, Jin Kyu and Lee, Seunghak and Ganger, Gregory R and Gibson, Garth and Keeton, Kimberly and Xing, Eric},
  booktitle={HotOS'2013},
  year={2013}
}

@inproceedings{suri,
  title={Counting triangles and the curse of the last reducer},
  author={Suri, Siddharth and Vassilvitskii, Sergei},
  booktitle={WWW'2011},
  pages={607--614},
  year={2011}
}

@inproceedings{GrayTransactionConcept,
  title={The transaction concept: Virtues and limitations},
  author={Gray, Jim and others},
  booktitle={VLDB},
  volume={81},
  pages={144--154},
  year={1981}
}

@inproceedings{recht2011hogwild,
	title={Hogwild: A lock-free approach to parallelizing stochastic gradient descent},
	author={Recht, Benjamin and Re, Christopher and Wright, Stephen and Niu, Feng},
	booktitle={NIPS'2011},
	pages={693--701},
	year={2011}
}

@book{BeHaGo87,
  title={Concurrency control and recovery in database systems},
  author={Bernstein, Philip A and Hadzilacos, Vassos and Goodman, Nathan},
  volume={370},
  year={1987},
  publisher={Addison-wesley, New York}
}

@article{EswaranGrayLorieTraiger1976,
  title={The notions of consistency and predicate locks in a database system},
  author={Eswaran, Kapali P. and Gray, Jim N and Lorie, Raymond A. and Traiger, Irving L.},
  journal={Communications of the ACM},
  volume={19},
  number={11},
  pages={624--633},
  year={1976},
  publisher={ACM}
}

@book{bertsekas1989parallel,
  title={Parallel and distributed computation: numerical methods},
  author={Bertsekas, Dimitri P and Tsitsiklis, John N},
  volume={23},
  year={1989},
  publisher={Prentice hall Englewood Cliffs, NJ}
}

@inproceedings{kogan2009predicting,
  title={Predicting risk from financial reports with regression},
  author={Kogan, Shimon and Levin, Dimitry and Routledge, Bryan R and Sagi, Jacob S and Smith, Noah A},
  booktitle={Proceedings of Human Language Technologies: The 2009 Annual Conference of the North American Chapter of the Association for Computational Linguistics},
  pages={272--280},
  year={2009},
  organization={Association for Computational Linguistics}
}

@inproceedings{avron2014revisiting,
  title={Revisiting asynchronous linear solvers: Provable convergence rate through randomization},
  author={Avron, Haim and Druinsky, Alex and Gupta, Anshul},
  booktitle={IPDPS'2014},
  pages={198--207},
  year={2014},
  organization={IEEE}
}

@article{frommer2000asynchronous,
  title={On asynchronous iterations},
  author={Frommer, Andreas and Szyld, Daniel B},
  journal={Journal of computational and applied mathematics},
  volume={123},
  number={1},
  pages={201--216},
  year={2000},
  publisher={Elsevier}
}

@article{nomad,
  author    = {Hyokun Yun and
               Hsiang{-}Fu Yu and
               Cho{-}Jui Hsieh and
               S. V. N. Vishwanathan and
               Inderjit S. Dhillon},
  title     = {{NOMAD:} {N}onlocking, st{O}chastic {M}ulti-machine algorithm for {A}synchronous
               and {D}ecentralized matrix completion},
  journal   = {{PVLDB}},
  volume    = {7},
  number    = {11},
  pages     = {975--986},
  year      = {2014}
}

@article{DimmWitted,
  author    = {Ce Zhang and
               Christopher Re},
  title     = {{DimmWitted}: {A} {S}tudy of {M}ain-{M}emory {S}tatistical {A}nalytics},
  journal   = {{PVLDB}},
  volume    = {7},
  number    = {12},
  pages     = {1283--1294},
  year      = {2014}
}

@inproceedings{Dean2012nips,
  author    = {Jeffrey Dean and
               Greg Corrado and
               Rajat Monga and
               Kai Chen and
               Matthieu Devin and
               Quoc V. Le and
               Mark Z. Mao and
               Marc'Aurelio Ranzato and
               Andrew W. Senior and
               Paul A. Tucker and
               Ke Yang and
               Andrew Y. Ng},
  title     = {Large Scale Distributed Deep Networks},
  booktitle = {NIPS'2012},
  pages     = {1232--1240},
  year      = {2012}
}

@inproceedings{Smola2010nips,
  author    = {Martin Zinkevich and
               Markus Weimer and
               Alexander J. Smola and
               Lihong Li},
  title     = {Parallelized Stochastic Gradient Descent},
  booktitle = {NIPS'2010},
  pages     = {2595--2603},
  year      = {2010}
}

@inproceedings{Pan2013nips,
  author    = {Xinghao Pan and
               Joseph E. Gonzalez and
               Stefanie Jegelka and
               Tamara Broderick and
               Michael I. Jordan},
  title     = {Optimistic Concurrency Control for Distributed Unsupervised Learning},
  booktitle = {NIPS'2013},
  pages     = {1403--1411},
  year      = {2013}
}

@inproceedings{Garth2013nips,
  author    = {Qirong Ho and
               James Cipar and
               Henggang Cui and
               Seunghak Lee and
               Jin Kyu Kim and
               Phillip B. Gibbons and
               Garth A. Gibson and
               Gregory R. Ganger and
               Eric P. Xing},
  title     = {More Effective Distributed {ML} via a Stale Synchronous Parallel Parameter
               Server},
  booktitle = {NIPS'2013},
  pages     = {1223--1231},
  year      = {2013},
}

@article{GraphLab,
  author    = {Yucheng Low and
               Joseph E. Gonzalez and
               Aapo Kyrola and
               Danny Bickson and
               Carlos Guestrin and
               Joseph M. Hellerstein},
  title     = {GraphLab: {A} New Framework For Parallel Machine Learning},
  journal   = {CoRR},
  volume    = {abs/1408.2041},
  year      = {2014},
  url       = {http://arxiv.org/abs/1408.2041},
}

@article{boyd2011distributed,
  title={Distributed optimization and statistical learning via the alternating direction method of multipliers},
  author={Boyd, Stephen and Parikh, Neal and Chu, Eric and Peleato, Borja and Eckstein, Jonathan},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={3},
  number={1},
  pages={1--122},
  year={2011},
  publisher={Now Publishers Inc.}
}
